Do Coding Agents Still Need a Debugger? Frontier-Model-Based Fault Localization at the Accuracy Ceiling

Background: To localize a fault, a coding agent can reason from source code alone or use debugger assistance by running the program and stepping through it in an interactive debugger. While earlier agents struggled with static execution tracing and debugger operation, frontier LLMs have improved at both. Objective: We evaluate how accurately coding agents localize faults without tools across original and transformed programs, how much debugger assistance improves accuracy and at what cost, and how agents use it when optional. Methods: We seed 610 single-line faults into 144 LeetCodeDataset solutions and rewrite each faulty program with five recipes of behavior-preserving transformations. Agents based on Sol 6.1, Luna 6, and Qwen 3.8 localize each fault with no, optional, or encouraged debugger assistance. Results: Without tools, the agents localized 98.2 to 99.9% of faults in original and 96.7 to 99.9% in transformed programs, losing accuracy mainly where recipes restructured loops and conditions. Encouraged assistance removed 63% and 61% of Luna 6's and Qwen 3.8's remaining transformed errors (+2.1 and +1.3 percentage points) at 14.7 to 27.0 times the token use, while Sol 6.1 stayed at 99.9%. With optional assistance, Luna 6 and Qwen 3.8 still gained +1.5 and +1.3 points, though the agents used the interactive debugger in only 0.2 to 6.2% of runs. Conclusions: On short, precisely specified programs, current coding agents localize nearly all faults from source code alone, and debugger assistance removes most errors that remain. Given the choice, agents executed the program far more often than they stepped through it, yet kept most of the benefit.

==> generated/table-accuracy-rows.tex <==
Luna 6 & Untransformed & 98.2 & 98.1 & 98.9 &  & +0.7 [+0.2, +1.4] & \\
 & Transformed & 96.7 & 98.2 & 98.8 & $-$1.5 [$-$2.3, $-$0.6] & +2.1 [+1.4, +2.8] & +1.4 [+0.6, +2.1] \\
\midrule
Sol 6.1 & Untransformed & 99.9 & 99.8 & 99.8 &  & $-$0.1 [$-$0.3, +0.0] & \\
 & Transformed & 99.9 & 99.9 & 99.9 & +0.0 [$-$0.1, +0.0] & +0.0 [+0.0, +0.1] & +0.1 [+0.0, +0.3] \\
\midrule
Qwen 3.8 & Untransformed & 98.8 & 98.9 & 99.1 &  & +0.3 [$-$0.3, +1.1] & \\
 & Transformed & 97.9 & 99.1 & 99.2 & $-$0.9 [$-$1.6, $-$0.1] & +1.3 [+0.8, +1.8] & +1.0 [+0.1, +1.7] \\


==> generated/table-cost-rows.tex <==
Luna 6 & Tokens (thousands) & 1.4 & 2.2 & 41.8 & 2.0 & 3.3 & 55.0 & 29.7$\times$ & 27.0$\times$ \\
 & Wall time (s) & 5.9 & 4.5 & 41.2 & 7.5 & 6.4 & 47.0 & 7.0$\times$ & 6.2$\times$ \\
 & Cost (US\$ per 1,000 episodes) & 0.22 & 0.25 & 1.26 & 0.32 & 0.38 & 1.60 & 5.7$\times$ & 5.0$\times$ \\
\midrule
Sol 6.1 & Tokens (thousands) & 1.3 & 3.6 & 25.0 & 1.7 & 4.9 & 32.2 & 19.8$\times$ & 18.4$\times$ \\
 & Wall time (s) & 4.9 & 14.0 & 37.8 & 5.2 & 15.0 & 39.9 & 7.7$\times$ & 7.7$\times$ \\
 & Cost (US\$ per 1,000 episodes) & 2.86 & 4.35 & 11.81 & 3.41 & 5.30 & 13.98 & 4.1$\times$ & 4.1$\times$ \\
\midrule
Qwen 3.8 & Tokens (thousands) & 3.3 & 19.0 & 37.4 & 5.0 & 38.3 & 73.5 & 11.2$\times$ & 14.7$\times$ \\
 & Wall time (s) & 37.9 & 136.1 & 213.6 & 66.4 & 245.0 & 350.4 & 5.6$\times$ & 5.3$\times$ \\
 & Cost (US\$ per 1,000 episodes) & 4.76 & 11.60 & 15.68 & 7.65 & 18.92 & 26.06 & 3.3$\times$ & 3.4$\times$ \\


==> generated/table-discretionary-rows.tex <==
\multicolumn{5}{@{}l}{\emph{Luna~6}} \\
\enspace Untr. & $-$0.1 [$-$1.0, +0.7] & $-$0.8 [$-$1.6, $-$0.2] & +3.2$^\dagger$ & -- \\
\enspace Transf. & +1.5 [+0.9, +2.2] & $-$0.6 [$-$1.0, $-$0.2] & +15.0$^\dagger$ & +66.7$^\dagger$ \\
\midrule
\multicolumn{5}{@{}l}{\emph{Sol~6.1}} \\
\enspace Untr. & $-$0.2 [$-$0.4, +0.0] & $-$0.1 [$-$0.2, +0.0] & $-$1.1$^\dagger$ & -- \\
\enspace Transf. & +0.0 [$-$0.1, +0.0] & +0.0 [$-$0.2, +0.0] & +0.0 [+0.0, +0.1] & $-$0.1 [$-$0.2, +0.0] \\
\midrule
\multicolumn{5}{@{}l}{\emph{Qwen~3.8}} \\
\enspace Untr. & +0.2 [$-$0.3, +0.7] & $-$0.2 [$-$0.7, +0.3] & +1.9 [$-$1.0, +5.5] & $-$0.7 [$-$2.1, +0.7] \\
\enspace Transf. & +1.3 [+0.8, +1.8] & +0.0 [$-$0.3, +0.2] & +5.3 [+3.2, +7.5] & +2.7$^\dagger$ \\


==> generated/table-programs-rows.tex <==
\multicolumn{8}{@{}l}{\emph{Reference programs}} \\
\quad Easy & 50 & 50 & 8 & \iqr{4--11} & 3 & \iqr{2--4} &  \\
\quad Medium & 48 & 50 & 11 & \iqr{7--14} & 4 & \iqr{3--5} &  \\
\quad Hard & 46 & 50 & 19 & \iqr{14--24} & 8 & \iqr{5--11} &  \\
\midrule
\multicolumn{8}{@{}l}{\emph{Faulty programs, by fault type}} \\
\quad Off-by-one & 125 & 150 & 13 & \iqr{9--18} & 5 & \iqr{3--7} &  \\
\quad Wrong arithmetic & 104 & 150 & 13 & \iqr{9--18} & 5 & \iqr{3--8} &  \\
\quad Wrong logic & 108 & 150 & 14 & \iqr{10--19} & 5 & \iqr{4--8} &  \\
\quad Wrong variable & 132 & 150 & 12 & \iqr{9--18} & 4 & \iqr{3--7} &  \\
\quad Static return & 141 & 150 & 12 & \iqr{8--18} & 4 & \iqr{3--7} &  \\
\midrule
\multicolumn{8}{@{}l}{\emph{Transformed programs, change by recipe}} \\
\quad Rename & 584 & 610 & +0\% & \iqr{0--0} & +0 & \iqr{0--0} & 40\% \\
\quad State \& literals & 610 & 610 & +71\% & \iqr{50--100} & +0 & \iqr{0--0} & 49\% \\
\quad Control flow & 610 & 610 & +169\% & \iqr{103--234} & +1 & \iqr{1--2} & 51\% \\
\quad Distractors & 610 & 610 & +400\% & \iqr{377--429} & +11 & \iqr{8--15} & 71\% \\
\quad Maximal mix & 608 & 610 & +450\% & \iqr{347--601} & +5 & \iqr{3--8} & 37\% \\


==> generated/table-tool-use-rows.tex <==
Luna 6 & Any debugger action & 0.0\% & 0.3\% & 100.0\% & 100.0\% \\
 & Probe runs only & 8.8\% & 11.8\% & 0.0\% & 0.0\% \\
 & Debugger actions & 0.0 & 0.0 & 11.6 & 12.5 \\
 & Probe runs & 0.1 & 0.2 & 1.1 & 1.2 \\
 & Breakpoints & -- & 18.4\% & 14.6\% & 17.5\% \\
 & Stepping & -- & 27.6\% & 45.8\% & 41.7\% \\
 & State inspection & -- & 13.2\% & 18.8\% & 16.0\% \\
\midrule
Sol 6.1 & Any debugger action & 0.0\% & 0.2\% & 100.0\% & 100.0\% \\
 & Probe runs only & 86.7\% & 98.4\% & 0.0\% & 0.0\% \\
 & Debugger actions & 0.0 & 0.0 & 8.0 & 8.4 \\
 & Probe runs & 0.9 & 1.0 & 1.1 & 1.1 \\
 & Breakpoints & -- & 23.1\% & 20.1\% & 21.3\% \\
 & Stepping & -- & 23.1\% & 45.5\% & 44.0\% \\
 & State inspection & -- & 17.9\% & 19.7\% & 20.2\% \\
\midrule
Qwen 3.8 & Any debugger action & 0.9\% & 6.2\% & 20.2\% & 41.7\% \\
 & Probe runs only & 99.1\% & 93.6\% & 79.8\% & 58.1\% \\
 & Debugger actions & 0.1 & 0.4 & 1.5 & 3.1 \\
 & Probe runs & 1.8 & 2.2 & 2.3 & 2.7 \\
 & Breakpoints & 31.5\% & 26.1\% & 22.6\% & 26.1\% \\
 & Stepping & 17.8\% & 19.2\% & 27.3\% & 22.9\% \\
 & State inspection & 8.2\% & 11.6\% & 13.4\% & 12.4\% \\

